Exploring Post Quantum Cryptography with Quantum Key Distribution for Sustainable Mobile Network Architecture Design

The proliferation of mobile networks and their increasing importance to modern life, combined with the emerging threat of quantum computing, present new challenges and opportunities for cybersecurity. This paper addresses the complexity of protecting these critical infrastructures against future quantum attacks while considering operational sustainability. We begin with an overview of the current landscape, identify the main vulnerabilities in mobile networks, and evaluate existing security solutions with new post-quantum cryptography (PQC) methods. We then present a quantum-secure architecture with PQC and Quantum Key Distribution (QKD) tailored explicitly for sustainable mobile networks and illustrate its applicability with several use cases that emphasize the need for advanced protection measures in this new era. In addition, a comprehensive analysis of PQC algorithm families is presented, focusing on their suitability for integration in mobile environments, with particular attention to the trade-offs between energy consumption and security improvements. Finally, recommendations for strengthening mobile networks against quantum threats are provided through a detailed examination of current challenges and opportunities.

==> prelim.tex <==
\subsection{PQC}

With advances in quantum computing technology, there is a risk that traditional cryptographic methods such as RSA and ECC will be broken, as quantum computers can efficiently solve certain mathematical problems on which these systems are based. In the context of mobile networks, where security and efficiency are paramount, PQC offers a promising solution to address the vulnerabilities of quantum computing. Post-quantum cryptography (PQC) could potentially close several security gaps in mobile transport networks, particularly with regard to the security of cryptographic algorithms against attacks by quantum computers \cite{ulitzsch2022post}. The PQC algorithms are designed to withstand attacks from both classical and quantum computers. By using PQC in mobile networks, operators can ensure that sensitive data transmitted over these networks remains secure in the face of future advances in quantum computing. Mobile networks are  also expected to have a long lifespan, and the data transmitted over them may need to remain secure for decades. The PQC algorithms are developed with long-term security in mind and provide robust protection against quantum attacks for many years to come. While early iterations of PQC algorithms may have been computationally intensive, ongoing research aims to optimize these algorithms for efficiency. This is particularly important for mobile networks where resources such as battery life and bandwidth are limited. As PQC algorithms continue to improve, their performance overhead in mobile environments is expected to decrease. Standardization bodies and industry organizations are actively working to develop and promote PQC algorithms that are suitable for various applications, including those in mobile networks. These concerted efforts ensure interoperability and facilitate the widespread adoption of PQC on different mobile platforms and devices.



At the end of a six-year process, \ac{NIST} selected the CRYSTALS-Kyber \cite{avanzi2019crystals} for general public key encryption and the three algorithms CRYSTALS-Dilithium, FALCON and SPHINCS+ for digital signature algorithms as primary standards\footnote{Online: https://www.nist.gov/news-events/news/2022/07/nist-announces-first-four-quantum-resistant-cryptographic-algorithms, Available: February 2024.}. The Falcon algorithm for digital signatures was selected as the standard for situations in which the use of Dilithium would be too complex.  Although, in the 3rd round of the NIST PQC competition, Kyber was selected for standardization, NIST is now assessing BIKE, Classic McEliece, HQC and SIKE in the 4th round.


\subsection{QKD}

Quantum Key Distribution (QKD) is a new approach to secure communication that uses the principles of quantum mechanics to provide a theoretically unbreakable encryption method. Unlike conventional cryptographic techniques that rely on computational complexity for security, QKD uses the quantum properties of particles, such as photons, to enable two parties to securely generate and exchange a cryptographic key. The use of quantum keys in symmetric encryption can significantly increase the security of communication systems. Any eavesdropping attempt disturbs the quantum state of these particles. This reveals the presence of an eavesdropper and ensures the integrity of the key.  Its integration into mobile network architectures is particularly important given the ubiquitous and sensitive nature of the data transmitted over these networks. 

